On Detecting Policy-Related Political Ads: An Exploratory Analysis of Meta Ads in 2022 French Election

Online political advertising has become the cornerstone of political campaigns. The budget spent solely on political advertising in the U.S. has increased by more than 100% from \$700 million during the 2017-2018 U.S. election cycle to \$1.6 billion during the 2020 U.S. presidential elections. Naturally, the capacity offered by online platforms to micro-target ads with political content has been worrying lawmakers, journalists, and online platforms, especially after the 2016 U.S. presidential election, where Cambridge Analytica has targeted voters with political ads congruent with their personality To curb such risks, both online platforms and regulators (through the DSA act proposed by the European Commission) have agreed that researchers, journalists, and civil society need to be able to scrutinize the political ads running on large online platforms. Consequently, online platforms such as Meta and Google have implemented Ad Libraries that contain information about all political ads running on their platforms. This is the first step on a long path. Due to the volume of available data, it is impossible to go through these ads manually, and we now need automated methods and tools to assist in the scrutiny of political ads. In this paper, we focus on political ads that are related to policy. Understanding which policies politicians or organizations promote and to whom is essential in determining dishonest representations. This paper proposes automated methods based on pre-trained models to classify ads in 14 main policy groups identified by the Comparative Agenda Project (CAP). We discuss several inherent challenges that arise. Finally, we analyze policy-related ads featured on Meta platforms during the 2022 French presidential elections period.

==> background.tex <==
\section{Background}
\label{background}
%\subsection{Automated analysis of political discourse}


\subsection{NLP approaches for political discourse analysis}
Identifying political topics in social media messages is a current problem and generates more and more research. By solving it, researchers can gain more knowledge about the difference in the popularity of specific issues for different candidates and a better understanding of various parties' strategies. One of the main pitfalls of this task is the lack of labeled data. 

To solve this problem \cite{terechshenko} the first article proposed to use the transfer learning approach, in which knowledge gained in the source area or task is transferred to another target area or task. They study the performance of language models by comparing them with various text classification methods. The authors used the CAP bills dataset as training data and CAP New York Times headlines for a test. They evaluated three machine learning classifiers: linear SVM, logistic regression, random forest, and three pre-trained models: ULMFIT, RoBERTa, and XL-Net. RoBERTa achieved the highest accuracy score (61\%). These results proved the possibility of using transfer learning for political science problems.

Authors of the next paper were also concerned about lack of training data for supervised classification and  proposed using a lexicon-based approach to solve this problem, where they built a list of language cues for nine political topics \cite{jackson}. 
For developing and testing their method, the authors used three datasets that were collected during the 2015-2016 U.S. election cycle
\begin{enumerate}
    \item Transcripts from 19 Republican and 9 Democratic primary debates.
    \item 29 thousand Facebook posts from Republican, Democratic, third parties presidential candidates.
    \item 98 million tweets from presidential candidates and people who mention them.
\end{enumerate}
Transcripts of primary debates were used to obtain seed words for a lexicon. Four annotators labeled fragments of the texts corresponding to one of nine topics. After that, the authors sorted labeled pieces of the texts into 18 documents for each topic for each party. For each document, the authors extracted all unigrams and bigrams, and next, two annotators familiar with U.S. politics checked ngrams and included them in the final lexicon for each topic. They used other datasets for lexicon revision and testing. This method performed well for eight topics out of 9.  

In opposite of a previous work, \cite{gupta2020polibert} used a supervised approach for topic characterization. The authors collected real-time tweets and Facebook's posts from 33 candidates during the period of 08/02/2015 to 11/10/2016 and after that split it into different categories (advocacy, attack, image, issue and e.t.c.). The resulting data set consists of 27,591 Facebook posts and 88,980 tweets from 33 candidates, that later were labeled for the training and test set. After using BERT classifier they achieved significant improvements for the multi-label classification task compared to Naive Bayes and SVM. 

\subsection{Meta Ad Library}
%%% delete or briefly mention 
In 2019, Meta launched the ad library \cite{metaadlibrary-2}, which allows its users to search for ads that are running on Meta services, and get details about the ads, including the funding entity, an indication of the amount spent, and the coverage of the ad across multiple demographics. In France, there are 4 advertising categories; real estate ads, employment ads, credit ads, and ads about social issues, elections, or politics. We are interested in the last type. 

According to Meta, an ad is deemed to be about  “social issues, elections or politics” if it is: \cite{meta2017}


\begin{itemize}
    \item “made by, on behalf of or about a candidate for public office, a political figure, a political party, a political action committee or advocates for the outcome of an election to public office; or
    \item about any election, referendum or ballot initiative, including "get out the vote" or election information campaigns; or
   \item is about any social issue in any place where the ad is being run; or
   \item is regulated as political advertising.”
\end{itemize}

Meta describes social issues as “highly politicized sensitive and heavily debated topics that polarize political opinion before elections” \cite{metaadlibrary-2}. Since most countries do not have laws or agencies which specify social issues that need to be regulated, the Ad library addresses a list of social issues for each country. The European Union's list includes civil and social rights, crime, economics, environmental policy, health, immigration, political values and governance, security, and foreign policy \cite{metaadlibrary-3}.

The Meta Ad Library performs using three major tools \cite{metaadlibrary-8}:

\begin{itemize}
    \item The Ad Library:  a web service offering a searchable collection of all ads currently active on Meta technologies (currently Facebook and Instagram) and all ads about social issues, elections, or politics that are also inactive. While political ads are stored in the library for seven years, non-political ones disappear once they are not active. \cite{metaadlibrary-5}
    \item The Meta Ad Library API : A programming interface that allows users to perform customized queries to retrieve all active and inactive ads about social issues, elections, or politics. \cite{metaadlibrary-6}
    \item The Meta Ad Library Report: groups advertisers' data for all ads about social issues, elections, or politics including spending totals, spending by specific advertisers, and spending data by geographic location. \cite{metaadlibrary-7}
\end{itemize}

\subsection{Online political advertising in France}
%%%% section 6
France’s presidential elections proceed in two rounds. On April 10, 2022, the first stage of voting narrowed the field of candidates from twelve to two; the second round, between outgoing President Emmanuel Macron and National Rally party’s Marine Le Pen, took place on April 24. On the other hand, legislative elections will be held on June 12 and 19, 2022, two months after the presidential election. They are held every five years.

France placed several legislative and soft law developments to regulate online political advertising. Law L.-52-1 of the Electoral Code states that in the six months preceding an election (presidential, legislative and senatorial, European, and referendums), the use of any commercial advertising through the press or by any means of audiovisual tools for electoral propaganda purposes is prohibited \cite{law-Electoral}. %Thus, the ads featured on Meta targeting French regions may be mainly discussing social issues. In addition, after analyzing our collected data, we notice that the official candidates do not fund any political ads, except for Emmanuel Macron, Marine Le Pen, and Eric Zemmour.


==> misc.tex <==
\section{Misc comments}
\oana{@oana: election principles to be respected -- fair representation
one of the key principles of any election systems is fair representaiton. Fair representation has been interepreted in different ways~\cite{XX},  need access to data that is fair 
The basic task for an electoral system is to translate votes into seats; to transform the expressed will of the voters into people who will represent it. There are many views of what fair representation is ? geographic representation, descriptive representation, ideological or party political representation ? but regardless of the view that is taken in each country, representation as a principle is a key guide when designing the most suitable electoral system.}
 
\oana{@oana: Need for audits on what it is said. }

\oana{@oana: many anecdotal examples -- not good in political communications} \oana{maybe cite own work on the diversity of issues that are talked about}

\oana{@oana: we need to make the case somewhere that politicla communications research needs this}

\oana{@oana: Additional: talk somewhere about: la couverture mediatiique and legislation in europe}


\update{
Although we do not consider accuracy as an evaluation metric, we will calculate it in a rather different way from the multi-class classification. We will only consider the category that has the highest prediction score. A true positive means that the predicted category is one of the labeled categories.
Total of tested ads = 735 
Total of true positive  = 566
\textbf{Accuracy = 77\%}}


4.2 \oana{can we sum up the overlap in one number? } 



\oana{additional analysis: (1) do ads about certain policy categories cost more than other categories? -- do a table like 10 but with the cost (2) do ads that talk about certain politicians cost more than other politicians? (3) compare macron end le pen before round 1 and before round 2 -- did they change their policy attention?}


==> model_evaluation_backup.tex <==
%!TEX root = paper.tex
\section{Model evaluation}
\label{sec:model_eval}

\subsection{Testing procedure}

The goal of this section is to find the configuration of the most accurate policy category classifier \update{and understand where the limits come from.} 
For some policy categories we are very limited in labeled data \footnote{Because some policy categories were less frequent in the input dataset (see Section~\ref{data})}, hence, to test the accuracy of the different classifiers in ``good'' conditions, we build and test classifiers only on 9 policy categories with more than 200 labeled ads: environment, international affairs, energy, civil rights, government operations, health, social policy, cultural policy and economy which includes foreign trade, macroeconomic policy and economic regulations. At the end of the section, once the ``winner'' configuration is identified, we analyze the accuracy of the classifier over the 14 policy categories: we added categories that have more (or close to) 100 labeled ads and less than 200. 

%\update{In the first step, a classification in 9 categories will be made taking into consideration the social issues having at least 200 labeled ads. Due to a lack of annotated data, we take only ads about these 9 categories and fine-tune our models on them. We cite: Environment, international affairs, energy, civil rights, government operations, health, social policy, cultural policy and economy which includes foreign trade, macroeconomic policyand economic regulations.} %Subsequently, 5 other categories will be added to the classification.}

To compare classifiers we evaluate their accuracy over the same test dataset that contains \xx ads whos labels represents the majority vote of Prolific workers (the \testn). In addition, we also evaluate the classifiers over a test dataset that contains \xx ads with labels provided by the domain experts (the \testgs -- see Section~\ref{XX}). \oana{introduce the dataset names in section 2} 

%\update{ 
%Due to the lack of data for some classes, we consider two instantiations of the dataset: one with 9 social issues (\vmd-9) and one with 14 social issues (Pub-14).}

\oana{discuss how you compute accuracy over multiple categories.}

micro-average of precision, recall and F1 score of the 9 categories. 




\subsection{Influence of the model architecture}

Table~\ref{tab:classificationResultGlobal} compares the accuracy of the fours types of models we investigate (i.e., SVM, Random Forest, FlauBERT and CamamBERT) to classify ads from \testn  into the 9 policy categories. 
To train the four models we used the \vmd and we report the accuracy of the best configuration of each classifier. For training and validation we performed 10-fold cross validation over the remaining data in \vmd after excluding data part of \testn. 


%We first compare the accuracy
%After it, we compared classifiers trained and tested on the data from the same domain: \vmd dataset. 
%Table \ref{tab:classificationResultGlobal} presents the results of the classification of ads into 9 categories,
%according to different models:

%\begin{itemize}
%    \item SVM and Random Forest using TF/IDF trained on the \vmd dataset.
%    \item FlauBERTtunedSocialIssues is a fine-tuned FlauBERT model on the task of classifying political ads according to the social issue addressed using the \vmd dataset.
%    %\item FlauBERTsoftLabels is a fine-tuned FlauBERT model on the task of classifying political ads according to the social issue addressed using the second dataset \disd.
%    \item CamemBERTunedSocialIssues is a fine-tuned CamemBERT model on the task of classifying political ads according to the social issue addressed using the \vmd dataset.
%    %\item FlauBERTcap is a fine-tuned FlauBERT model on the task of classifying political ads according to the social issue addressed using the \textbf{CAP} dataset.
%\end{itemize}


\begin{table}[t]
\centering
\caption{Accuracy across models over \testn. The tables presents the micro-averages of precision, recall and F1 scores.}
%\resizebox{\columnwidth}{!}{
\small{
\begin{tabular}{lrrr}
    \toprule
    %& Micro average of precision & Micro average of recall  & Micro average of f1 scores   \\
    & Precision & Recall & F1\\
    \midrule
    SVM & 0.45 & 0.40 & 0.52 \\
    Random Forest & 0.39 &  0.33 & 0.46 \\
    FlauBERTtuned & \textbf{0.79} & \textbf{0.59} & \textbf{0.68} \\
    %FlauBERTsoftLabels & \textbf{0.79} & \textbf{0.60}  & \textbf{0.68} \\
    CamemBERTtuned & 0.72 & 0.61 & 0.66 \\
    %FlauBERTcap & 0.14 & 0.11 & 0.13 \\
    \bottomrule
    \end{tabular}
    }
%  \vspace{-2cm}
\label{tab:classificationResultGlobal}
\end{table}
%\FloatBarrier

The F1 score shows that our tuned versions of FlauBERT and CamemBERT significantly outperform SVM and Random Forest and are able to achieve F1 scores over 0.65. 
%When analysing the f1 score obtained, we observe that language models robustly outperform the other models tested. 
As expected, models that use both pre-trained language models and task-tailored language models for feature extraction generally perform better than TF/IDF methods. 
Supervised models perform worse as they can only exploit our small quantities of labeled data. SVM slightly outperforms Random Forest, which is expected as it is known it performs better with small quantities of labeled data. 
\oana{this interpretation is booring, remove?}



\subsection{Influence of the training data}
In the following, we continue with the FlauBERTtuned model as it has slightly outperformed CamemBERTtuned.


The previous section used the \vmd to train models. In this section, we first investigate whether a transfer learning approach would work by using the \capd to train FlauBERT. The advantage of using \capd is that it contains 25.4k labeled examples which is more than the number of our labeled ads.  
Table~\ref{tab:classificationResultsoftlabels} presents the accuracy and we see that FlauBERTcap is able to achieve only a 0,13 F1 score. Hence, transfer learning does not work in our case. We hypothesise that this difference might be because the \capd contains test that is linguistically different than political ads posted on Meta, or that texts from CAP are single labeled whereas our ads are multi-labeled which may confuse the model. \oana{I do not understand the idea behind this, why single labels will confuse the classifier?} 
\update{Despite the large number of CAP texts that have been annotated, they have an average length of 36 words. Thus, a text may not carry information to the models.} \oana{I do not see the link between the lenght and not cary enough informaiton}


 

%Since, we have more labeled data in CAP dataset, initially we decided to try transfer-learning approach. FlauBERT model were fine-tuned on the task of classifying political ads according to the social issue addressed using the \textbf{CAP} dataset (FlauBERTcap).

%\begin{table}[H]
%%\centering
%\caption{Results of the classification of ads according to 9 categories: transfer learning}
%%\resizebox{\columnwidth}{!}{
%\begin{tabular}{lrrr}
%    \toprule
%    & Precision & Recall & F1\\
%    \midrule
%    FlauBERTcap & 0.14 & 0.11 & 0.13 \\
%    \bottomrule
%    \end{tabular}
%\label{tab:classificationResultCAP}
%\end{table}

Previous works have showed that soft labels might help the classification task as extra data. Hence, to understand how disagreement between annotators can influence classification results, we fine-tuned FlauBERT model on the task of classifying political ads according to the policy category  using the second dataset \disd (FlauBERTsoftLabels).
\oana{so you train on both \vmd and \disd or just \disd?}

\begin{table}[t]
\centering
\caption{Accuracy across training dataset. Comparison of FlauBERT's accuracy trained with \capd, \vmd (majority vote labels), and \disd (soft labels).}
%\resizebox{\columnwidth}{!}{
\small{
\begin{tabular}{lrrr}
    \toprule
    %& Micro average of precision & Micro average of recall  & Micro average of f1 scores   \\
    & Precision & Recall & F1\\
    \midrule
        FlauBERTcap & 0.14 & 0.11 & 0.13 \\
    FlauBERTtuned & 0.79 & 0.59 & 0.68\\
    FlauBERTsoftLabels & 0.79& 0.60& 0.68\\
    \bottomrule
    \end{tabular}
    }
\label{tab:classificationResultsoftlabels}
\end{table}

Table~\ref{tab:classificationResultsoftlabels} shows that the F1 score of FlauBERTsoftLabels does not improve on the F1 score of FlauBERTtuned. 
Taking into account the disagreements between annotators does not have a great influence on the accuracy of the results. \update{We can conclude that the categories chosen by the voting majority  represent well the social issues addressed in the ad message.} \oana{are you sure our results can be use to conclude this?}


\subsection{Influence of the policy categories }
Figure \ref{tab:test-9cat-th} illustrates the precision, recall and F1 score of FlauBERTtuned across the 9 policy categories. The support is the number of texts in a specific category in the test set. The table shows that the accuracy to identify some policy categories such as  \textit{environment, energy} and \textit{cultural policy} is much higher than the accuracy if identifying ads related to \textit{social policy}. 

To dig the root cause, Figure~\ref{XX} shows a heat-map of the overlap between different policy categories. We can observe that the policy categories with high overlap, lead to lower accuracy. \oana{explain why this leads to lower accuracy}


\begin{table}[t]
\caption{Accuracy across policy categories using FlauBERTtuned over \testn.}
% \begin{tabular}{ |p{2cm}| p{1cm}| p{1cm} |p{1cm} |p{1cm}| }
%     \hline
%   &precision & recall & f-1 score &support  \\\hline
% International affairs & 0.81 & 0.60 & 0.69&100 \\\hline
% \rowcolor{bittersweet}Energy & 0.93 &0.68&0.79&100 \\\hline
% Government operations & 0.65 & 0.43&0.52&105\\\hline
% \rowcolor{bittersweet}Cultural policy & 0.84 & 0.83&0.83&109\\\hline
% \rowcolor{ballblue}Social policy &0.76& 0.19&0.30&102\\\hline
% Health&0.86&0.73&0.79&102\\\hline
% Human rights, civil liberties and discrimination& 0.67&0.47&0.55&125\\\hline
% \rowcolor{bittersweet}Environment&0.81&0.80&0.81&150\\\hline
% Economic&0.75&0.49&0.59&102\\\hline
% micro avg&0.79&0.59&0.68&995\\\hline
% macro avg&0.79&0.58&0.65&995\\\hline
% weighted avg& 0.79&0.59&0.66&995\\\hline
% samples avg&0.72&0.64&0.66&995\\\hline
% \end{tabular}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
    \toprule
    &Prec. & Rec. & F-1 & support  \\
    \midrule
    International affairs & 0.81 & 0.60 & 0.69&100 \\
    \rowcolor{bittersweet}Energy & 0.93 &0.68&0.79&100 \\
    Government operations & 0.65 & 0.43&0.52&105\\
    \rowcolor{bittersweet}Cultural policy & 0.84 & 0.83&0.83&109\\
    \rowcolor{ballblue}Social policy &0.76& 0.19&0.30&102\\
    Health&0.86&0.73&0.79&102\\
    Human rights, civil liberties and discrimination& 0.67&0.47&0.55&125\\
    \rowcolor{bittersweet}Environment&0.81&0.80&0.81&150\\
    Economy&0.75&0.49&0.59&102\\
    \midrule
    micro avg&0.79&0.59&0.68&995\\
%    macro avg&0.79&0.58&0.65&995\\
%    weighted avg& 0.79&0.59&0.66&995\\
%    samples avg&0.72&0.64&0.66&995\\
    \bottomrule
\end{tabular}}
\label{tab:test-9cat-th}
\end{table}
%\begin{figure}[hbt!]
%  \centering
%  \includegraphics[width=8cm]{images/test_9cat_th.PNG}
%  \caption{Classification report of test data according to 9 categories using FlauBERTtunedSocialIssues. \textbf{Threshold = 0.5}.}
%  \label{fig:test-9cat-th}
%\end{figure}
%\FloatBarrier

\subsection{Influence of the number of policy categories}

The previous section showed that the overlap in content between policy categories has a nefarious impact on the achievable accuracy. In this section we look at how accuracy changes when we consider more policy categories. Here we train and test classifiers using 14 policy categories for which we have more than 100 ads. We add the following policy categories: \textit{education, justice and crime, work and employment, urban and territorial policies}, and \textit{immigration.} Unfortunately, we do not have enough labeled data to add the \xx other categories.
Table~\ref{tab:test-14cat-th} shows the accuracy across the 14 policy categories. The table shows that even for policy categories such as \xx and \xx for which we have less than 200 ads, the classifier is able to achieve F1 scores over \xx. The table also shows that the accuracy of the initial 9 policy categories slightly drops. This can be explained by the fact that increasing the number of categories will also lead to higher overlaps between policy categories. \oana{can we sum up the overlap in one number? } 


%Figure \ref{tab:test-14cat-th} and \ref{tab:test-14cat-tho} illustrate the classification report of test data using the 14 categories classifier FlauBERTtunedSocialIssues.



\begin{table}[t]
\centering
\caption{Accuracy across policy categories using FlauBERTtuned over the \testf.}
\resizebox{\columnwidth}{!}{
% \begin{tabular}{ |p{2cm}| p{1cm}| p{1cm} |p{1cm} |p{1cm}| }
%     \hline
%   &precision & recall & f-1 score &support  \\\hline
% International affairs & 0.68 & 0.49 & 0.57&102 \\\hline
% Energy & 0.92 &0.59&0.72&100 \\\hline
% Immigration&0.71&0.50&0.59&30\\\hline
% Law and crime&0.83&0.29&0.43&35\\\hline
% Government operations & 0.64 & 0.41&0.50&105\\\hline
% Cultural policy & 0.83& 0.71&0.76&110\\\hline
% Social policy & 0.85& 0.11&0.19&104\\\hline
% Urban and territorial policies&0.61&0.45&0.52&31\\\hline
% Health&0.85&0.67&0.75&101\\\hline
% Labor and employment & 0.59&0.61&0.60&36\\\hline
% Human rights, civil liberties and discrimination& 0.63&0.51&0.57&134\\\hline
% Education&0.88&0.23&0.36&31\\\hline
% Environment & 0.76& 0.79&0.78&150\\\hline
% Economy&0.89&0.23&0.37&103\\\hline
% micro avg&0.75&0.50&0.60&1172\\\hline
% macro avg&0.76&0.47&0.55&1172\\\hline
% weighted avg& 0.77&0.50&0.58&1172\\\hline
% samples avg&0.64&0.56&0.58&1172\\\hline
% \end{tabular}
\begin{tabular}{lrrrr}
    \toprule
  &Prec. & Rec. & F-1 &support  \\
  \midrule
International affairs & 0.68 & 0.49 & 0.57&102 \\
Energy & 0.92 &0.59&0.72&100 \\
Immigration&0.71&0.50&0.59&30\\
Law and crime&0.83&0.29&0.43&35\\
Government operations & 0.64 & 0.41&0.50&105\\
Cultural policy & 0.83& 0.71&0.76&110\\
Social policy & 0.85& 0.11&0.19&104\\
Urban and territorial policies&0.61&0.45&0.52&31\\
Health&0.85&0.67&0.75&101\\
Labor and employment & 0.59&0.61&0.60&36\\
Human rights, civil liberties and discrimination& 0.63&0.51&0.57&134\\
Education&0.88&0.23&0.36&31\\
Environment & 0.76& 0.79&0.78&150\\
Economy&0.89&0.23&0.37&103\\
\midrule
micro avg&0.75&0.50&0.60&1172\\
%macro avg&0.76&0.47&0.55&1172\\
%weighted avg& 0.77&0.50&0.58&1172\\
%samples avg&0.64&0.56&0.58&1172\\
\bottomrule
\end{tabular}
\label{tab:test-14cat-th}}
\end{table}


%\begin{figure}[hbt!]
%  \centering
%  \includegraphics[width=8cm]{images/test_14cat_th.PNG}
%  \caption{Classification report of test data according to 14 categories using FlauBERTtunedSocialIssues. \textbf{Threshold = 0.5}.}
%  \label{fig:test-14cat-th}
%\end{figure}
%\FloatBarrier






\subsection{Final model configuration}
For using a policy category in a classifier, it is important to minimise false positive in the detriment of false negatives--it is more important not to mislabel ads with the wrong policy category than missing some ads that are related to a policy category. Hence to give more priority to precision than recall. Given this preference, instead of using the same threshold for each category (i.e., 0.5), we select a different threshold for each policy category. 

To get the appropriate threshold for each category we performed \textit{threshold optimization} as a fine-tuning step. The definition of the threshold is done during the validation phase by maximizing precision over recall. We, therefore, look for thresholds that give a precision close to 85\% with the highest possible recall. The threshold optimization process is as follows.  

%The last layer of the model returns scores for each text (network input); these scores are between 0 and 1 and represent the probability that the text belongs to a certain category; the higher the score, the higher the probability that a text belongs to a category. 
%
%Once we have obtained the output score  \textit{\(s_{ij}\)} for a specific ad \textit{i} and category \textit{j}, we needed to find a threshold \(t_j\) to convert \textit{\(s_{ij}\)} into label predictions \(y_{ij}\) 
%in \(y\) . Here,  \(y_{ij}\) can be expressed as follows:  \(y_{ij} = 1\) (if \(s_{ij} > t_j\) ) . 
%Let \textit{\(s_{11}\)}, be the probability of the first ad to address the category \textit{environment}, which if its value is greater than  \(t_1\), the prediction \(y_{11}\) is 1 and 0 otherwise, representing whether or not this advertisement discusses the social issue \textit{environment}.
%The threshold is usually set at 0.5 in binary classifications. 
%
%After obtaining the output scores \textit{s} for the ads in the validation set, we compute the metrics: recall, precision and f1\_score per category considering several threshold values. Then, we select for each category the threshold that gives us a precision close to 85\% and a recall as high as possible. 

Table~\ref{tab:test-14cat-tho} presents the precision and recall of FlauBERtuned with 14 policy categories using different thresholds.  Note that the precision is not always close to 0.85 since the thresholds have been defined on validation data and not on test data.  In the next section we use this model for label prediction. 

%\begin{table}[H]
%\caption{Classification report of test data according to 9 categories using FlauBERTtunedSocialIssues. \textbf{Different threshold were taken per category.}}
%\resizebox{\columnwidth}{!}{
%% \begin{tabular}{ |p{2cm}| p{1cm}| p{1cm} |p{1cm} |p{1cm}| }
%%     \hline
%%   &precision & recall & f-1 score &support  \\\hline
%% International affairs & 0.76 & 0.64 & 0.70&100 \\\hline
%% Energy & 0.91 &0.74&0.82&100 \\\hline
%% Government operations & 0.71 & 0.19&0.30&105\\\hline
%% Cultural policy & 0.85& 0.78&0.81&109\\\hline
%% Social policy & 0.86& 0.06&0.11&102\\\hline
%% Health&0.88&0.34&0.49&102\\\hline
%% Human rights, civil liberties and discrimination& 0.89&0.40&0.50&125\\\hline
%% Environment & 0.83& 0.73&0.78&150\\\hline
%% Economy&0.89&0.40&0.55&102\\\hline
%% micro avg&0.84&0.47&0.60&995\\\hline
%% macro avg&0.84&0.46&0.55&995\\\hline
%% weighted avg& 0.84&0.47&0.56&995\\\hline
%% samples avg&0.60&0.52&0.54&995\\\hline
%\begin{tabular}{lrrrr}
%  \toprule
%  &Prec. & Rec. & f-1  & support  \\
%  \midrule
%International affairs & 0.76 & 0.64 & 0.70&100 \\
%Energy & 0.91 &0.74&0.82&100 \\
%Government operations & 0.71 & 0.19&0.30&105\\
%Cultural policy & 0.85& 0.78&0.81&109\\
%Social policy & 0.86& 0.06&0.11&102\\
%Health&0.88&0.34&0.49&102\\
%Human rights, civil liberties and discrimination& 0.89&0.40&0.50&125\\
%Environment & 0.83& 0.73&0.78&150\\
%Economy&0.89&0.40&0.55&102\\
%\midrule
%micro avg&0.84&0.47&0.60&995\\
%macro avg&0.84&0.46&0.55&995\\
%weighted avg& 0.84&0.47&0.56&995\\
%samples avg&0.60&0.52&0.54&995\\
%\bottomrule
%\end{tabular}}
%\label{tab:test-9cat-tho}
%\end{table}
%%\begin{figure}[hbt!]
%% \centering
%%  \includegraphics[width=8cm]{images/test_9cat_tho.PNG}
%%  \caption{Classification report of test data according to 9 categories using FlauBERTtunedSocialIssues. \textbf{Different threshold were taken per category.}}
%%  \label{fig:test-9cat-tho}
%%\end{figure}
%%\FloatBarrier

\update{
Although we do not consider accuracy as an evaluation metric, we will calculate it in a rather different way from the multi-class classification. We will only consider the category that has the highest prediction score. A true positive means that the predicted category is one of the labeled categories.
Total of tested ads = 735 
Total of true positive  = 566
\textbf{Accuracy = 77\%}}


\begin{table}[t]
\centering
\caption{Accuracy across policy categories using FlauBERTtuned over the \testf. \textbf{Different thresholds per category.}}

% \begin{tabular}{ |p{2cm}| p{1cm}| p{1cm} |p{1cm} |p{1cm}| }
%     \hline
%   &precision & recall & f-1 score &support  \\\hline
% International affairs & 0.93 & 0.26 & 0.41&102 \\\hline
% Energy & 0.96 &0.45&0.61&100 \\\hline
% Immigration&0.57&0.27&0.36&30\\\hline
% Law and crime&0.75&0.26&0.38&35\\\hline
% Government operations & 0.73 & 0.21&0.33&105\\\hline
% Cultural policy & 0.78& 0.75&0.76&110\\\hline
% Social policy & 0.76& 0.12&0.21&104\\\hline
% Urban and territorial policies&0.89&0.26&0.40&31\\\hline
% Health&0.84&0.60&0.70&101\\\hline
% Labor and employment & 1&0.17&0.29&36\\\hline
% Human rights, civil liberties and discrimination& 0.79&0.20&0.32&134\\\hline
% Education&0.75&0.29&0.42&31\\\hline
% Environment & 0.79& 0.71&0.75&150\\\hline
% Economy&0.89&0.16&0.26&103\\\hline
% micro avg&0.81&0.38&0.51&1172\\\hline
% macro avg&0.82&0.34&0.44&1172\\\hline
% weighted avg&0.82& 0.38&0.48&1172\\\hline
% samples avg&0.52&0.43&0.46&1172\\\hline
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
    \toprule
  &Prec. & Rec. & F-1 score &support  \\
  \midrule
International affairs & 0.93 & 0.26 & 0.41&102 \\
Energy & 0.96 &0.45&0.61&100 \\
Immigration&0.57&0.27&0.36&30\\
Law and crime&0.75&0.26&0.38&35\\
Government operations & 0.73 & 0.21&0.33&105\\
Cultural policy & 0.78& 0.75&0.76&110\\
Social policy & 0.76& 0.12&0.21&104\\
Urban and territorial policies&0.89&0.26&0.40&31\\
Health&0.84&0.60&0.70&101\\
Labor and employment & 1&0.17&0.29&36\\
Human rights, civil liberties and discrimination& 0.79&0.20&0.32&134\\
Education&0.75&0.29&0.42&31\\
Environment & 0.79& 0.71&0.75&150\\
Economy&0.89&0.16&0.26&103\\
\midrule
micro avg&0.81&0.38&0.51&1172\\
%macro avg&0.82&0.34&0.44&1172\\
%weighted avg&0.82& 0.38&0.48&1172\\
%samples avg&0.52&0.43&0.46&1172\\
\bottomrule
\end{tabular}
}
\label{tab:test-14cat-tho}
\end{table}

%We chose FlauBERTtunedSocialIssues for 14 categories with different thresholds per category as our final model. In the next section, we use it for label prediction. 



%\begin{figure}[hbt!]
%  \centering
%  \includegraphics[width=8cm]{images/test_14cat_tho.PNG}
%  \caption{Classification report of test data according to 14 categories using FlauBERTtunedSocialIssues. \textbf{Different threshold were taken per category.}}
%  \label{fig:test-14cat-tho}
%\end{figure}
%\FloatBarrier

% \subsection{Difficulty of the task}


% After visualizing our results and realizing the complexity of the task, we wanted to investigate the quality of our labels. To do so, we label ourselves 50\% of the test data, which we call golden labels, and then compare them with the labels of the Prolific annotators. The figure shows the classification ratio assuming that our golden labels are the real labels and the prolific labels are predictions. The goal is to show the difference between the labels.

% \begin{table}[H]
% \centering
% \caption{Classification report according to 9 categories between gold labels and Prolific labels}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lrrrr}
%     \toprule
%   &Prec. & Rec. & f-1 & support  \\
%   \midrule
% International affairs & 0.61 & 0.74 & 0.67&50 \\
% Energy & 0.77 &0.81&0.79&68 \\
% Government operations & 0.74 & 0.58&0.65&85\\
% Cultural policy & 0.84& 0.65&0.73&80\\
% Social policy & 0.39& 0.56&0.46&48\\
% Health&0.68&0.77&0.72&56\\
% Human rights, civil liberties and discrimination& 0.45&0.78&0.57&149\\
% Environment & 0.62& 0.78&0.69&78\\
% Economy&0.40&0.45&0.42&53\\
% \midrule
% micro avg&0.61&0.68&0.64&567\\
% macro avg&0.61&0.68&0.55&567\\
% weighted avg& 0.64&0.68&0.56&567\\
% samples avg&0.66&0.70&0.65&567\\
% \bottomrule
% \end{tabular}}
% \label{tab:test-classificationReportGold}
% \end{table}
%\begin{figure}[hbt!]
%  \centering
%  \includegraphics[width=8cm]{images/test_goldLabels.PNG}
%  \caption{Classification report according to 9 categories between gold labels and Prolific labels}
%  \label{fig:test-classificationReportGold}
%\end{figure}
%\FloatBarrier


% According to figure \ref{tab:classificationResultGlobal}, there is a disagreement between our annotations and those of Prolific. The annotators on Prolific have a time constraint that needs to be respected. Thus, some social issues might be ignored by the annotated seeing our list have 26 social issues. In our case, we have no time limitation, although we concluded that it is sometimes difficult to label ads according to social issue. Let's take this ad as an example: "A donation can save thousands of Ukrainians". It may be considered as addressing social policy by some people, while another person may assign human rights as the issue addressed. This difficulty in defining social issues, in addition to the minimal amount of data used, can justify the rather limited performance of the models.
